Direct numerical simulations of ripples in an oscillatory flow

Sea ripples are small-scale bedforms which originate from the interaction of an oscillatory flow with an erodible sand bed. The phenomenon of sea ripple formation is investigated by means of direct numerical simulation in which the sediment bed is represented by a large number of fully-resolved spherical grains. Two sets of parameter values are adopted which are motivated by laboratory experiments on the formation of laminar rolling-grain ripples. The knowledge on the origin of ripples is presently enriched by insights and by providing fluid- and sediment-related quantities that are difficult to obtain in the laboratory. Detailed analysis of flow and sediment bed evolution has confirmed that ripple wavelength is determined by the action of steady recirculating cells which tend to accumulate sediment grains into ripple crests. The ripple amplitude is observed to grow exponentially consistent with established linear stability analysis theories. Particles at the bed surface exhibit two kinds of motion depending on their position with respect to the recirculating cells: particles at ripple crests are significantly faster and show larger excursions than those lying on ripple troughs. In analogy with segregation phenomenon of polydisperse sediments the non-uniform distribution of the velocity field promotes the formation of ripples. The wider the gap between the excursion of fast and slow particles, the the larger the resulting growth rate of ripples. Finally, it is revealed that, in the absence of turbulence, the sediment flow rate is driven by both the bed shear stress and the wave-induced pressure gradient, the dominance of each depending on the phase of the oscillation period. In phases of maximum bed shear stress, the sediment flow rate correlates more with the Shields number while the pressure gradient tends to drive sediment bed motion during phases of minimum bed shear stress.

==> nomenclature.tex <==
%\input{symbol_cmd.tex}
%=====================================================================
%               NOMENCLATURE
%
\nomenclature{\mob}{Mobility number}
%
\nomenclature{\Rdel}{Stokes Reynolds number}
%
\nomenclature{\Rd}{Particle Reynolds number}
%
\nomenclature{\Ga}{Galileo number}
%
\nomenclature{\Kc}{Keulegan-Carpenter number}
%
\nomenclature{\denss}{Grain density}
%
\nomenclature{\densf}{Fluid density}
%
\nomenclature{\g}{Gravitational acceleration}
%
\nomenclature{\ds}{Sphere diameter}
%
\nomenclature{\s}{Relative density}
%
\nomenclature{\U}{Free-stream Velocity}
%
\nomenclature{\kvis}{Kinematic viscosity of the fluid}
%
\nomenclature{\dvis}{Dynamic viscosity of the fluid}
%
\nomenclature{\del}{Conventional Stokes boundary layer thickness}
%
\nomenclature{\om}{Angular frequency of flow oscillations}
%
\nomenclature{\TT}{Oscillation period}
%
\nomenclature{$t$}{Time variable}
%
\nomenclature{(\vc{x}{})}{Cartesian coordinates}
%
\nomenclature{(\vc{u}{})}{Fluid velocity components}
%
\nomenclature{(\vc{f}{})}{Eulerian volume force components}
%
\nomenclature{$p$}{Pressure}
%
\nomenclature{\svf}{Solid volume fraction}
%
\nomenclature{\svfm}{Maximum solid volume fraction}
%
\nomenclature{\bsur}{Bed surface}
%
\nomenclature{\bprP}{Bed profile - definition 1}
%
\nomenclature{\bprPrms}{rms of bed profile}
%
\nomenclature{\bprE}{Bed profile - definition 2}
%
\nomenclature{$\sav{\cdot}_{\vc{x}{}}$}{Space average}
%
\nomenclature{$\sav{\cdot}_{s}$}{Particle average}
%
\nomenclature{$\sav{\cdot}_{T}$}{Half-period average}
%
\nomenclature{$\tav{\cdot}$}{Time average}
%
%\nomenclature{$\pav{\cdot}$}{Phase average}
%
\nomenclature{\wln}{Dominant wavelength of ripples}
%
\nomenclature{\wlns}{Dominant wavelength of the steady streaming close to the bed}
%
\nomenclature{\pse}{Particle semi-excursion}
%
%\nomenclature{$u_{is}, i=1,2,3$}{Particle velocity}
%
%\nomenclature{$F_{is}, i=1,2,3$}{Particle force}
%
\nomenclature{\fse}{Fluid semi-excursion}
%
\nomenclature{\prf}{Particle reference force}
%
\nomenclature{\phs}{Transport initiation phase for top-particles}
%
\nomenclature{\tin{}}{Start phase of particle tracking}
%
\nomenclature{(\pvc{u}{})}{Particle velocity components}
%
%\nomenclature{(\pvc{\Omega}{})}{Particle rotation velocity components}
%
\nomenclature{(\pvc{F}{})}{Particle force components}
%
\nomenclature{(\pvc{T}{})}{Particle torque components}
%
\nomenclature{\Npt}{Number of particles}
%
\nomenclature{\SSp}{Spatial spectrum}
%
\nomenclature{\sstr}{Magnitude of the steady streaming}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%% STYLE %%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\nomlabel}[1]{#1\hfil} % To shift the first column to the right
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% AMAN
\nomenclature{\tautot}{Total shear stress}
%
\nomenclature{\tauf}{Fluid shear stress}
%
\nomenclature{\taup}{Particle shear stress}
%
\nomenclature{\shields}{Shields number}
%
\nomenclature{\qpmean}{Mean particle flow rate}
%
\nomenclature{\qref}{Inertial flow rate scale} 
%
%=====================================================================
